Waveform Simulation for Scintillation Characteristics of NaI(Tl) Crystal

The lowering of the energy threshold in the NaI detector is crucial not only for comprehensive validation of DAMA/LIBRA but also for exploring new possibilities in the search for low-mass dark matter and observing coherent elastic scattering between neutrino and nucleus. Alongside hardware enhancements, extensive efforts have focused on refining event selection to discern noise, achieved through parameter development and the application of machine learning. Acquiring pure, unbiased datasets is crucial in this endeavor, for which a waveform simulation was developed. The simulation data were compared with the experimental data using several pulse shape discrimination parameters to test its performance in describing the experimental data. Additionally, we present the outcomes of multi-variable machine learning trained with simulation data as a scintillation signal sample. The distributions of outcomes for experimental and simulation data show a good agreement. As an application of the waveform simulation, we validate the trigger efficiency alongside estimations derived from the minimally biased measurement data.

==> Makefile <==
main:
	pdflatex WFSim

full:
	pdflatex WFSim
	bibtex WFSim
	pdflatex WFSim
	pdflatex WFSim

submit:
	sed -f submit.sed < WFSim.tex > WFSim_submit.tex
	pdflatex WFSim_submit
	pdflatex WFSim_submit

clean:
	rm *-converted-to.pdf *.aux *.bbl *.blg *.dvi *.log *.toc *.lof *.lot *.out *.fdb* *.fls *~ \#*\# *Notes.bib *.spl *.gz *.pdf

